Parallel Independence in Attributed Graph Rewriting

In order to define graph transformations by the simultaneous application of concurrent rules, we have adopted in previous work a structure of attributed graphs stable by unions. We analyze the consequences on parallel independence, a property that characterizes the possibility to resort to sequential rewriting. This property turns out to depend not only on the left-hand side of rules, as in algebraic approaches to graph rewriting, but also on their right-hand side. It is then shown that, of three possible definitions of parallel rewriting, only one is convenient in the light of parallel independence.

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{P. Bahr (Ed.): 11th International Workshop on\\
Computing with Terms and Graphs (TERMGRAPH 2020)\\
EPTCS 334, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.334.5}{10.4204/EPTCS.334.5}}

